S/C: Speeding up Data Materialization with Bounded Memory

With data pipeline tools and the expressiveness of SQL, managing interdependent materialized views (MVs) are becoming increasingly easy. These MVs are updated repeatedly upon new data ingestion (e.g., daily), from which database admins can observe performance metrics (e.g., refresh time of each MV, size on disk) in a consistent way for different types of updates (full vs. incremental) and for different systems (single node, distributed, cloud-hosted). One missed opportunity is that existing data systems treat those MV updates as independent SQL statements without fully exploiting their dependency information and performance metrics. However, if we know that the result of a SQL statement will be consumed immediately after for subsequent operations, those subsequent operations do not have to wait until the early results are fully materialized on storage because the results are already readily available in memory. Of course, this may come at a cost because keeping results in memory (even temporarily) will reduce the amount of available memory; thus, our decision should be careful. In this paper, we introduce a new system, called S/C, which tackles this problem through efficient creation and update of a set of MVs with acyclic dependencies among them. S/C judiciously uses bounded memory to reduce end-to-end MV refresh time by short-circuiting expensive reads and writes; S/C's objective function accurately estimates time savings from keeping intermediate data in memory for particular periods. Our solution jointly optimizes an MV refresh order, what data to keep in memory, and when to release data from memory. At a high level, S/C still materializes all data exactly as defined in MV definitions; thus, it doesn't impact any service-level agreements. In our experiments with TPC-DS datasets (up to 1TB), we show S/C's optimization can speedup end-to-end runtime by 1.04x-5.08x with 1.6GB memory.

==> header/ccs.tex <==
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10002951.10002952.10003212.10003213</concept_id>
       <concept_desc>Information systems~Database utilities and tools</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10002951.10002952.10003190.10003205</concept_id>
       <concept_desc>Information systems~Database views</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Information systems~Database utilities and tools}
\ccsdesc[500]{Information systems~Database views}
%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.

==> header/vldbstuff.tex <==
%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\pagestyle{\vldbpagestyle}
\begingroup\small\noindent\raggedright\textbf{PVLDB Reference Format:}\\
\vldbauthors. \vldbtitle. PVLDB, \vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
\endgroup
\begingroup
\renewcommand\thefootnote{}\footnote{\noindent
This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
\raggedright Proceedings of the VLDB Endowment, Vol. \vldbvolume, No. \vldbissue\ %
ISSN 2150-8097. \\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
}\addtocounter{footnote}{-1}\endgroup
%%% VLDB block end %%%

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\ifdefempty{\vldbavailabilityurl}{}{
\vspace{.3cm}
\begingroup\small\noindent\raggedright\textbf{PVLDB Artifact Availability:}\\
The source code, data, and/or other artifacts have been made available at \url{\vldbavailabilityurl}.
\endgroup
}
%%% VLDB block end %%%

==> sections/plots/ours_vs_no_opt.tex <==
%!TEX root = main.tex

\begin{figure*}[t]

\pgfplotsset{accfig/.style={
    width=90mm,
    height=50mm,
    legend columns=5,
    every axis/.append style={font=\footnotesize},
    % ymajorgrids,
    % yminorgrids,
    minor grid style=lightgray,
    % nodes near coords,
    % every node near coord/.append style={font=\footnotesize,anchor=west,rotate=60}
}}

\pgfplotsset{timefig/.style={
    width=58mm,
    height=35mm,
    xmin=10,
    xmax=100,
    ymin=0,
    ymax=60,
    xlabel=Number of Queries,
    ylabel=Runtime (sec),
    xlabel near ticks,
    ylabel near ticks,
    ylabel style={align=center},
    xtick={0, 10, ..., 100},
    % xticklabels={80\%, 85\%, 90\%, 95\%, 99\%, 99.5\%},
    ytick={0, 10, ..., 60},
    % yticklabels={0\%, 10\%, 20\%, 30\%},
    % xticklabel style={rotate=30,yshift=-2mm,anchor=east,xshift=1.5mm},
    % yticklabels={0 hr, 0.5 hr, 1 hr, 1.5 hr, 2.0 hr},
    % extra y ticks={10, 20, 30, 40},
    % extra y tick style={yticklabels={}},
    ylabel shift=-2pt,
    xlabel shift=-2pt,
    legend style={
        at={(0,1.15)},anchor=south west,column sep=2pt,
        draw=black,fill=none,line width=.5pt,
        /tikz/every even column/.append style={column sep=5pt}
    },
    legend columns=4,
    every axis/.append style={font=\footnotesize},
    % ymajorgrids,
    % yminorgrids,
    minor grid style=lightgray,
    % nodes near coords,
    % every node near coord/.append style={font=\footnotesize,anchor=west,rotate=60}
}}

\begin{subfigure}[b]{0.96\linewidth}
\begin{tikzpicture}
\begin{axis}[accfig,
    ybar,
    bar width=1.2mm,
    xlabel=RMS Error,
    xmin=0.5,
    xmax=5.5,
    xtick={1, 2, ..., 5},
    xticklabels={Job 1, Job 2, Job 3, Job 4, Job 5},
    ylabel=Time (ms),
    ymin=1,
    ymax=600,
    ytick={100, 200, 300, 400, 500, 600},
    yticklabels={100, 200, 300, 400, 500, 600},
    xticklabel style={yshift=2mm},
    xlabel style={yshift=0mm},
    xtick style={draw=none},
    legend style={
        at={(1.0,1.1)},anchor=south east,column sep=2pt,
        draw=black,fill=white,line width=.5pt,
        /tikz/every even column/.append style={column sep=5pt}
    },
    legend columns=4,
    area legend,
    clip=false,
    ymajorgrids,
    % yminorgrids,
    ylabel shift=-4pt,
    ]

% No Memory
\addplot[
thick,draw=vintagegreen,fill=vintagegreen,
]
table[x=x,y=y] {
x y
1 353.672
2 65.734
3 539.266
4 151.718
5 306.163
};

% 8GB Memory
\addplot[
thick,draw=vintageorange,fill=vintageorange,
]
table[x=x,y=y] {
x y
1 268.877
2 64.408
3 541.616
4 150.532
5 269.597
};

% 16GB Memory
\addplot[
thick,draw=vintageorange,fill=vintageorange,
]
table[x=x,y=y] {
x y
1 266.361
2 64.407
3 447.216
4 114.764
5 259.06
};

% 32GB Memory
\addplot[
thick,draw=vintageorange,fill=vintageorange,
]
table[x=x,y=y] {
x y
1 185.925
2 64.407
3 361.805
4 114.763
5 190.967
};

% \node[anchor=north west,draw=black,align=left,fill=white] at (axis cs: 0.6, 500000) {dataset: \dmv};

% \addlegendentry{STHoles}
\addlegendentry{$M =$ 0}
% \addlegendentry{ISOMER+QP}
\addlegendentry{$M =$ 8GB}
\addlegendentry{$M =$ 16GB}
\addlegendentry{$M =$ 32GB}

% \node[draw=black!50!vintagegreen,fill=white,font=\small,anchor=north east]
%   at (axis cs: 4.8,52) {2400 sec};

\end{axis}
\end{tikzpicture}

\vspace{-2mm}
\caption{Error vs.~Time}
\label{fig:exp:perf:c}
\end{subfigure}

\caption{
Comparison between  and
query-driven histograms. 
The lower, the better.
% The errors are the absolute errors of selectivity estimates in root-mean-square (rms). 
Left: 
The per-query overhead of 
was extremely low. Middle:  was the most accurate for the same time budget.
% \emph{(note: QueryModel's error reached 8,793\% for \insta)}.
Right:  required significantly less time for the same accuracy.
}
% The top row is for the \dmv dataset; the bottom row is for the \insta dataset.
\label{fig:exp:acc}
\end{figure*}

